Capability-based Frameworks for Industrial Robot Skills: a Survey

The research community is puzzled with words like skill, action, atomic unit and others when describing robots' capabilities. However, for giving the possibility to integrate capabilities in industrial scenarios, a standardization of these descriptions is necessary. This work uses a structured review approach to identify commonalities and differences in the research community of robots' skill frameworks. Through this method, 210 papers were analyzed and three main results were obtained. First, the vast majority of authors agree on a taxonomy based on task, skill and primitive. Second, the most investigated robots' capabilities are pick and place. Third, industrial oriented applications focus more on simple robots' capabilities with fixed parameters while ensuring safety aspects. Therefore, this work emphasizes that a taxonomy based on task, skill and primitives should be used by future works to align with existing literature. Moreover, further research is needed in the industrial domain for parametric robots' capabilities while ensuring safety.

==> structure.tex <==
\subsection{CLASSIFICATION OF PAPERS}

[proposal] classification of the papers could be done as follows:
\begin{itemize}
    \item \sout{skill definition [DEF]}
    \item skill hierarchy [HIER]:
    \begin{itemize}
        \item 1: SkillClass: Backhaus, Huckaby and then check the table [TE]
        \item 2: Skills: Pedersen, Zech, Andersen, Profanter, Backhaus [TE]
        \item 4: ParametrizedSkills: Profanter [TE]
        
        \item 3: Primitives: Pedersen, Andersen [MP]
        \item 5: Task: Pedersen  [MP]
        \item 6: Process: Backhaus, Huckaby [MP]
        
        \item 7: Request: NOT NECESSARY FOR NOW
    \end{itemize}
    \item skills integration framework [ARCH]: high level architecture of how skills can communicate and be integrated
    \item skill implementation [IMPL]: a clear example of how the skill was implemented on the robot focusing on the framework used (e.g. PLCopen blocks as state machine, a whole script running on ROS etc..)
    \item skill parameters/features [PARAM]
\end{itemize}


\section{Systematic reviews}

Limit to the latest 20 year

Keywords:
- Robot skills
- Industrial/Manufacturing
- Task
- (Collaborative) not mandatory


Simply use the section and subsection commands, as in this example document! With Overleaf, all the formatting and numbering is handled automatically according to the template you've chosen. If you're using Rich Text mode, you can also create new section and subsections via the buttons in the editor toolbar.


1. Description of the classes with schema and the example to see how we would do the classification?

Sub-section: How the review was conducted on the previous? a BAsic principle

2. Do we extract one definition of classes (skills, primitive, task etcc..?) and how this was done?

Take the 5 most important papers and create the definitions

3. Analysis on the papers:

1 Hierarchy representation

In our case our hierarchy is as follows and other authors do as follows

2 Human collaborative aspects (params)

Which representations should we have for this? Are there representations that do not fit well to collab robots

3 Features regarding the technological adoption (IND vs non-IND)

Technological features, Implemented, Parameters, Name derivation (from standard or from authors)

Different approaches are there but which are the skills really adopted and limiting factors

4. Direction of future works (evidence of this with an example, how a technology could be evaluated?)

Which features we should more work: what are we still missing from the actual contributions
